ShapeFormer: Shape Prior Visible-to-Amodal Transformer-based Amodal Instance Segmentation

Amodal Instance Segmentation (AIS) presents a challenging task as it involves predicting both visible and occluded parts of objects within images. Existing AIS methods rely on a bidirectional approach, encompassing both the transition from amodal features to visible features (amodal-to-visible) and from visible features to amodal features (visible-to-amodal). Our observation shows that the utilization of amodal features through the amodal-to-visible can confuse the visible features due to the extra information of occluded/hidden segments not presented in visible display. Consequently, this compromised quality of visible features during the subsequent visible-to-amodal transition. To tackle this issue, we introduce ShapeFormer, a decoupled Transformer-based model with a visible-to-amodal transition. It facilitates the explicit relationship between output segmentations and avoids the need for amodal-to-visible transitions. ShapeFormer comprises three key modules: (i) Visible-Occluding Mask Head for predicting visible segmentation with occlusion awareness, (ii) Shape-Prior Amodal Mask Head for predicting amodal and occluded masks, and (iii) Category-Specific Shape Prior Retriever aims to provide shape prior knowledge. Comprehensive experiments and extensive ablation studies across various AIS benchmarks demonstrate the effectiveness of our ShapeFormer. The code is available at: \url{https://github.com/UARK-AICV/ShapeFormer}

==> tabs/L_a.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.50\textwidth}{!}{
    \begin{tabular}{c|c|cccc|cccc}
    \toprule
        \multirow{2}{*}{$L_a$} & \multirow{2}{*}{\# \textbf{Params}} & \multicolumn{4}{c|}{\textbf{KINS}}& \multicolumn{4}{c}{\textbf{COCOA}} \\
        ~ & ~ & $AP$ & $AP_{50}$ & $AP_{75}$ & $AR$ & $AP$ & $AP_{50}$ & $AP_{75}$ & $AR$ \\\midrule
        1 & 1.6M & 34.05 & 58.61 & 35.74 & 22.04 & 35.68 & 62.70 & 36.64 & 9.93 \\ 
        2 & 3.2M & 34.02 & 58.43 & 35.78 & 23.89 & 35.51 & 62.44 & 36.54 & 9.81 \\ 
        3 & 4.8M & 33.87 & 58.43 & 35.92 & 22.04 & 35.90 & 62.35 & 36.61 & 9.85 \\ 
        4 & 6.4M & 34.14 & 58.70 & 35.65 & 22.13 & 35.63 & 62.41 & 36.72 & 9.91 \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{Ablation study on the number of layers ($L_a$) in Amodal Transformer Decoder. For each specified number of $L_a$, both amodal segmentation performances and the number of params required by Vis-Occ Transformer Decoder are reported}
    \label{abla:La}
\end{table}

==> tabs/L_v.tex <==
\begin{table}[!h]
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{c|c|cccc|cccc}
    \toprule
        \multirow{2}{*}{$L_v$} & \multirow{2}{*}{\# \textbf{Params}} & \multicolumn{4}{c|}{\textbf{KINS}}& \multicolumn{4}{c}{\textbf{COCOA}} \\
        ~ & ~ & $AP$ & $AP_{50}$ & $AP_{75}$ & $AR$ & $AP$ & $AP_{50}$ & $AP_{75}$ & $AR$ \\ \midrule
        1 & 1.6M & 31.08 & 53.89 & 32.14 & 21.01 & 32.56 & 57.83 & 33.91 & 9.33 \\ 
        2 & 3.2M & 31.31 & 54.33 & 32.57 & 21.13 & 33.18 & 58.32 & 34.50 & 9.44 \\ 
        3 & 4.8M & 31.29 & 55.01 & 31.98 & 21.11 & 33.01 & 58.21 & 34.65 & 9.41 \\ 
        4 & 6.4M & 31.62 & 55.81 & 31.47 & 21.14 & 33.31 & 58.42 & 34.78 & 9.50 \\ \bottomrule
    \end{tabular}
    }
    \caption{Ablation study on the number layers $L_v$ in Vis-Occ Transformer Decoder $\mathcal{D}_v$. For each specified number of $L_v$, both visible segmentation performances and the number of params required by Vis-Occ Transformer Decoder are reported.} 
    \label{abla:Lv}
\end{table}

==> tabs/abla_mask_attn_cocoa.tex <==
\begin{table}[!t]
    \caption{Impact of SP mask-attention (masked attn.) in amodal transformer decoder $\mathcal{D}_a$ on COCOA.}
    \centering
    \setlength{\tabcolsep}{6pt}
    \resizebox{0.40\textwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Dataset} & \shortstack{\textbf{SP masked attn.}}& $AP$ & $AP_{50}$ & $AP_{75}$ & $AR$ \\ \midrule
        \multirow{2}{*}{{\shortstack{COCOA}}} & \xmark     & 34.9 & 62.2 & 35.4 & 9.6 \\
        & \checkmark & \textbf{35.7} & \textbf{62.7} & \textbf{36.6} & \textbf{9.9} \\ \bottomrule
    \end{tabular}
    }
    \label{abla:masked_attention_cocoa}
    \vspace{-0.2cm}
\end{table}

==> tabs/aisformer_vs_shapeformer.tex <==
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{0.8}
\vspace{-0.4cm}
\caption{AISFormer and ShapeFormer comparison}
\vspace{-0.4cm}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|l|l|l}
            & amodal-to-visible & visible-to-amodal & Shape prior \\ \hline
AISFormer   & \checkmark        & \checkmark    & \xmark      \\
ShapeFormer & \xmark            & \checkmark    & \checkmark 
\end{tabular}
}
\label{tab:compare}
\vspace{-1em}
\end{table}

==> tabs/extend_vis2amodal.tex <==
\begin{table}[!h]
    \vspace{-0.3cm}
    \centering
    \caption{Impacts of Vis-to-Amodal on COCOA \& COCOA-cls}
    \vspace{-0.3cm}
    \resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|c|c|cc|cc|cc|cc}
    \toprule
        \multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\shortstack{visible\\to\\amodal}} & \multirow{3}{*}{\shortstack{amodal\\to\\visible}}& \multicolumn{4}{c|}{\textbf{COCOA-cls}} & \multicolumn{4}{c}{\textbf{COCOA}} \\ \cline{4-11}
        ~ & ~ &  ~ &\multicolumn{2}{c}{\textbf{Visible}} & \multicolumn{2}{c|}{\textbf{Amodal}} &  \multicolumn{2}{c}{\textbf{Visible}}& \multicolumn{2}{c}{\textbf{Amodal}}  \\ \cline{4-11}
         ~& ~ & ~ & AP & AR & AP & AR & AP & AR & AP & AR \\ \midrule
       Baseline           & \checkmark & \checkmark & 34.0 & 36.0 & 34.9 & 36.7 & 32.8 & 9.7 & 34.1 & 9.2 \\
Vis-Occ Mask Head  & \xmark     & \xmark     & 35.0 & 36.4 & -    & -    & 33.2 & 9.4 & -    & -   \\
ShapeFormer w/o SP & \checkmark & \xmark     & 35.0 & 36.4 & 35.8 & 37.1 & 33.2 & 9.4 & 34.9 & 9.6\\ \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \label{abla:vis2amodal_cocoa_cocoa_cls}
\end{table}

==> tabs/model_efficiency.tex <==
\begin{table}[!h]
\renewcommand{\arraystretch}{0.8}
\vspace{-1em}
\caption{Performance and network efficiency comparison with ResNet-50 as the backbone on KINS datasets.}
\vspace{-1em}
\label{tab:model_efficiency}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lll|llc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Performance}}                  & \multicolumn{3}{c}{\textbf{Complexity}}                                                                       \\ \cline{2-6} 
                        & \multicolumn{1}{c|}{AP $\uparrow$} & \multicolumn{1}{c|}{AR $\uparrow$} & \multicolumn{1}{c|}{Params $\downarrow$} & \multicolumn{1}{c|}{Inference time (FPS) $\uparrow$} & \multicolumn{1}{c}{GFLOPs$\downarrow$} \\ \hline
\multicolumn{1}{l|}{AISFormer}   & \multicolumn{1}{c|}{29.7} & \multicolumn{1}{c|}{33.8} & \multicolumn{1}{c|}{54.5M}  & \multicolumn{1}{c|}{13.3}      & 321                  \\
\multicolumn{1}{l|}{VRSP-Net}    & \multicolumn{1}{c|}{29.9} & \multicolumn{1}{c|}{32.1} & \multicolumn{1}{c|}{54.9M}  & \multicolumn{1}{c|}{12.9}      & 343                  \\ \midrule
\multicolumn{1}{l|}{\textbf{ShapeFormer}} & \multicolumn{1}{c|}{31.3} & \multicolumn{1}{c|}{34.1} & \multicolumn{1}{c|}{54.9M}  & \multicolumn{1}{c|}{13}        & 351       \\  \bottomrule
\vspace{-3.0em}     
\end{tabular}}
\end{table}

==> tabs/rebuttal_extended_exp.tex <==
\begin{table}[!h]
    \vspace{-0.3cm}
    \centering 
    \caption{Extended ablation study}
    \vspace{-0.3cm}
    \resizebox{1.0\linewidth}{!}{
    \setlength{\tabcolsep}{2pt}
    \subfloat[Extended visible-to-amodal ablation]{
    \resizebox{0.93\linewidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc}
    \toprule
       \multirow{3}{*}{\shortstack{visible\\to\\amodal}} & \multirow{3}{*}{\shortstack{amodal\\to\\visible}}& \multicolumn{4}{c|}{\textbf{COCOA-cls}} & \multicolumn{4}{c}{\textbf{COCOA}} \\ \cline{3-10}
         ~ &  ~ &\multicolumn{2}{c}{\textbf{Visible}} & \multicolumn{2}{c|}{\textbf{Amodal}} &  \multicolumn{2}{c}{\textbf{Visible}}& \multicolumn{2}{c}{\textbf{Amodal}}  \\ \cline{3-10}
         ~ & ~ & $AP\uparrow$ & $AR\uparrow$ & $AP\uparrow$ & $AR\uparrow$ & $AP\uparrow$ & $AR\uparrow$ & $AP\uparrow$ & $AR\uparrow$ \\ \midrule
        \checkmark & \checkmark & 34.0 & 36.0 & 34.9 & 36.7 & 32.8 & 9.7 & 34.1 & 9.2 \\
\xmark     & \xmark     & 35.0 & 36.4 & -    & -    & 33.2 & 9.4 & -    & -   \\
\checkmark & \xmark     & 35.0 & 36.4 & 35.8 & 37.1 & 33.2 & 9.4 & 34.9 & 9.6\\ \bottomrule
    \end{tabular}
    }
    }
    \quad
    \subfloat[Masked attention ablation.]{
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{ccccc}
        \toprule
        \multicolumn{5}{c}{\textbf{COCOA}} \\ \hline
        \shortstack{\textbf{SP}}& $AP\uparrow$ & $AP_{50}\uparrow$ & $AP_{75}\uparrow$ & $AR\uparrow$ \\ \midrule
         \xmark     & 34.9 & 62.2 & 35.4 & 9.6 \\
         \checkmark & \textbf{35.7} & \textbf{62.7} & \textbf{36.6} & \textbf{9.9} \\ \bottomrule
    \end{tabular}
    }
    }
    }
    \vspace{-0.7cm}
    \label{abla:extended_abla_exp}
\end{table}

==> tabs/rebuttal_vis-occ_variants.tex <==
\begin{table}[!h]
    \vspace{-1em}
    \renewcommand{\arraystretch}{0.8}
    \caption{\small ShapeFormer's visible prediction performance when Vis-Occ Mask Head is designed by CNN, GCN, and Transformer.}
    \vspace{-1em}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
    \toprule
        \multirow{2}{*}{\shortstack{Vis-Occ.\\ Mask Head}} & \multicolumn{4}{c|}{\textbf{KINS}} & \multicolumn{4}{c}{\textbf{COCOA}} \\ 
        ~ & $AP\uparrow$ & $AP_{50}\uparrow$ & $AP_{75}\uparrow$ & $AR\uparrow$ & $AP\uparrow$ & $AP_{50}\uparrow$ & $AP_{75}\uparrow$ & $AR\uparrow$ \\ \midrule
        CNN & $29.12$ & $50.48$ & $30.29$ & $20.70$ & $31.50$ & $56.25$ & $31.12$ & $9.33$ \\
        GCN & $30.46$ & $52.88$ & $32.02$ & $21.10$ & $33.26$ & $57.87$ & $33.97$ & $9.38$ \\ \midrule
        \textbf{Transformer} & \textbf{31.31} & \textbf{54.33} & $\textbf{32.57}$ & $\textbf{21.13}$ & $\textbf{34.00}$ & $\textbf{58.59}$ & $\textbf{35.90}$ & $\textbf{9.40}$  \\ \bottomrule
    \end{tabular}
    }
    \vspace{-1em}
    \label{abla:vis-occ-modeling}
\end{table}

